ATTIQA: Generalizable Image Quality Feature Extractor using Attribute-aware Pretraining

In no-reference image quality assessment (NR-IQA), the challenge of limited dataset sizes hampers the development of robust and generalizable models. Conventional methods address this issue by utilizing large datasets to extract rich representations for IQA. Also, some approaches propose vision language models (VLM) based IQA, but the domain gap between generic VLM and IQA constrains their scalability. In this work, we propose a novel pretraining framework that constructs a generalizable representation for IQA by selectively extracting quality-related knowledge from VLM and leveraging the scalability of large datasets. Specifically, we select optimal text prompts for five representative image quality attributes and use VLM to generate pseudo-labels. Numerous attribute-aware pseudo-labels can be generated with large image datasets, allowing our IQA model to learn rich representations about image quality. Our approach achieves state-of-the-art performance on multiple IQA datasets and exhibits remarkable generalization capabilities. Leveraging these strengths, we propose several applications, such as evaluating image generation models and training image enhancement models, demonstrating our model's real-world applicability.

==> Main/partials/figure_diffusion_user_study.tex <==
–\begin{figure}[t]
\centering
\includegraphics[clip, trim={1 0 0 0}, width=0.45 \textwidth]{Main/assets/diffusion_example.pdf}
\caption{Examples of generated images. The images are synthesized using the same prompt. ATTIQA hits human preference while others do not.}
\label{fig:diffusion}
\end{figure}


% % \usepackage[margin=0pt,labelformat=simple]{subcaption}
% \begin{figure}[t]
% \small
% \centering
% \begin{subfigure}[b]{0.45\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{Main/assets/r.pdf}
%     \caption{caption a.}
%     \label{fig:Teaser1}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.53\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{Main/assets/diffusion_user_study.pdf}
%     % \vspace{0.5pt}
%     \caption{caption b.}
%     \label{fig:Teaser2}
% \end{subfigure}
% \caption{fig1 caption}
% \label{fig:Teaser}
% \end{figure}


% \begin{subfigure}[b]{0.45\linewidth}
% \centering
% \includegraphics[clip, trim={0.3cm 0 0 0}, width=2 \linewidth]{Main/assets/diffusion_example.pdf}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.4\linewidth}
% \centering
%     \begin{tabular}{c||c|c|c}
%     \toprule
%     Method & CONTRIQUE & Re-IQA & ATTIQA \\
%     \midrule
%     Accuracy (\%) & 61.5 & 55.0 & \textbf{71.0} \\
%     \bottomrule
%     \end{tabular}
% \end{subfigure}

==> Main/partials/figure_enhancement_2.tex <==
% \begin{table}[htb]
% \centering
% \subfloat[Caption1]{%
% \resizebox{0.45\columnwidth}{!}{
%     }
% }
% \subfloat[Caption2]{%
%     \resizebox{0.515\columnwidth}{!}{
%     \begin{tabular}{c||c|c|c}
%     \toprule
%     Method & Expert C & Draw & Ours \\
%     \midrule
%     Human preference (\%) & 37.7 & 0.7 & \textbf{61.6}\\
%     \bottomrule
%     \end{tabular}
%     }
% }
% \caption{Overall table caption}
% \label{tab:mytable}
% \end{table}

\begin{figure}
  \begin{minipage}[b]{.45\linewidth}
    \centering
    \includegraphics[width=0.7\linewidth]{Main/assets/enhancement_user_study.pdf}
    \captionof{figure}{Figure caption}% \caption{Figure caption}
  \end{minipage}\hfill
  \begin{minipage}[b]{.45\linewidth}
    \centering
    \begin{tabular}{ *{5}{c} }
      A & b & C & d & e \\
      \hline
      1 & 2 & 3 & 4 & 5
    \end{tabular}
    \captionof{table}{Table caption}
  \end{minipage}
\end{figure}


==> Main/partials/figure_enhancement_user_study.tex <==
\begin{figure}[t]
\centering
\includegraphics[clip, trim={1 0 0 0}, width=0.35 \textwidth]{Main/assets/enhancement_user_study.pdf}
\caption{User study result of image enhancement}
\label{fig:enhancement_user_study}
\end{figure}



==> Main/partials/table_ablation.tex <==
\begin{table}[t]
\label{t3}
\begin{center}
\resizebox{\columnwidth}{!}
{
        \begin{tabular}{c||cc|cc|cc}
    \toprule
    \multirow{2}{*}{Prompt type}& \multicolumn{2}{c}{CLIVE} & \multicolumn{2}{c}{KonIQ} & \multicolumn{2}{c}{SPAQ}\\
    & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
    \midrule
    single-prompt & 0.880 & 0.909 & 0.928 & 0.939 & 0.916 & 0.920 \\
    Worst prompt & 0.869 & 0.889 & 0.930 & 0.943 & 0.920 & 0.925 \\
    Median prompt & 0.872 & 0.893 & 0.931 & 0.944 & 0.921 & 0.925 \\
    Hand-crafted & 0.896 & 0.914 & 0.940 & 0.950 & 0.925 & 0.929 \\
    \midrule
    with $L_2$ &  0.875 & 0.904 & 0.933 & 0.945 & 0.923 & 0.928 \\  
    \midrule
    ATTIQA & \textbf{0.898} & \textbf{0.916} & \textbf{0.942} & \textbf{0.952} & \textbf{0.926} & \textbf{0.930} \\
    \bottomrule
    \end{tabular}
}
\end{center}
\caption{Ablation study results.}
\label{table:ablation}
\end{table}

==> Main/partials/table_baselines.tex <==
\begin{table}[t]

\label{t3}
\begin{center}
\resizebox{\columnwidth}{!}
{


        \begin{tabular}{c||ccc}
    \toprule
    Methods & Contents aware & Distortion aware & Attribute aware \\
    \midrule
    HyperIQA & &\checkmark & \\
    CONTRIQUE & \checkmark & \checkmark & \\
    QPT & \checkmark & \checkmark & \\
    Re-IQA & \checkmark & \checkmark & \\
    \midrule
    Ours & & \checkmark & \checkmark \\
    \bottomrule
    \end{tabular}


}
\end{center}
\caption{Comparison with baselines.}
\label{table:baselines}
\end{table}

==> Main/partials/table_diffusion.tex <==
\begin{table}[t]

\label{t3}
\begin{center}
\resizebox{0.8\columnwidth}{!}
{

    \begin{tabular}{c||c|c|c}
    \toprule
    Method & CONTRIQUE & Re-IQA & ATTIQA \\
    \midrule
    Accuracy (\%) & 61.5 & 55.0 & \textbf{71.0} \\
    \bottomrule
    \end{tabular}

}
\end{center}
\caption{Comparisons of accuracy between human preferences and IQA model's result.}
\label{table:diffusion}
\end{table}

==> Main/partials/table_enhancement.tex <==
\begin{table}[t]

\label{t3}
\begin{center}
\resizebox{0.8\columnwidth}{!}
{

    \begin{tabular}{c||c|c|c}
    \toprule
    Method & Expert C & Draw & Ours \\
    \midrule
    Human preference (\%) & 37.7 & 0.7 & \textbf{61.6}\\
    \bottomrule
    \end{tabular}

}
\end{center}
\caption{Human preference comparison between our image enhancement model trained using ATTIQA's score and Expert C.}
\label{table:enhancement}
\end{table}

==> Main/partials/table_feature.tex <==
\begin{wraptable}{r}{0.5\columnwidth}
\label{t3} % here
\centering
\resizebox{0.5\columnwidth}{!}
{
    \centering
    \begin{tabular}{c||c|c|c}
    \toprule
     Fine-tune DB & CLIVE & KonIQ & SPAQ\\
    % \midrule
    %  Test DB & CLIVE & KonIQ & SPAQ & CLIVE & KonIQ & SPAQ & CLIVE & KonIQ & SPAQ \\
    \midrule
    \makecell{Re-IQA \\ (cosine similarity btw original $\leftrightarrow$ finetuned Re-IQA)} & 0.158 & 0.181  & 0.243\\
    \midrule
    \makecell{CONTRIQUE \\ (cosine similarity btw original $\leftrightarrow$ finetuned Re-IQA)} & 0.536 & 0.566 & 0.613\\
    \midrule
    \makecell{CLIP \\ (cosine similarity btw original $\leftrightarrow$ finetuned CLIP)} & 0.195 & 0.203  & 0.309\\
    \midrule
    \makecell{ATTIQA \\ (cosine similarity btw pretrained $\leftrightarrow$ finetuned ATTIQA)} & 0.890 & 0.811 & 0.945\\
    \bottomrule
    \end{tabular}  
}
\caption{
% Cosine similarity between features from pretrained and fine-tuned encoder.
A good generalization ability (\ie high cosine similarity) for IQA is obtained through our pretraining.}
\label{table:feature} % here
\end{wraptable}


==> Main/partials/table_generalization.tex <==
\begin{table}[htb]
    \begin{minipage}{0.5\columnwidth}
        \centering
       \caption{Linear probing performance comparison of ATTIQA and NR-IQA methods which focuses on representation learning.}
       \resizebox{\columnwidth}{!}{
            \begin{tabular}{c||cc|cc|cc}
            \toprule
            \multirow{2}{*}{Methods} & \multicolumn{2}{c}{CLIVE} & \multicolumn{2}{c}{KonIQ} & \multicolumn{2}{c}{SPAQ}\\
            & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
            \midrule
            CONTRIQUE & \underline{0.845} & \underline{0.857} & 0.894 & 0.906 & \underline{0.916} & 0.919 \\
            QPT & 0.761 & 0.794 & - & - & - & -\\
            Re-IQA (quality) & 0.806 & 0.824 & 0.861 & 0.885 & 0.900 & 0.910 \\
            Re-IQA (content) & 0.808 & 0.844 & 0.896 & 0.912 & 0.902 & 0.908 \\
            Re-IQA (both) & 0.840 & 0.854 & \textbf{0.914} & \textbf{0.923} & \textbf{0.918} & \textbf{0.925} \\
            CLIP & 0.803 & 0.829 & 0.883 & 0.895 & 0.895 & 0.896 \\
            \midrule
            ATTIQA & \textbf{0.870} & \textbf{0.891} & \underline{0.903} & \underline{0.918}  & \textbf{0.918} & \underline{0.922} \\
            \bottomrule
            \end{tabular}
        }
        \label{table:lp}
    \end{minipage}
    \begin{minipage}{0.44\columnwidth}
        \centering
        \caption{Cross dataset validation performance comparison of ATTIQA and existing NR-IQA methods.}
        \resizebox{\columnwidth}{!}{
            \begin{tabular}{c||cc|cc|cc}
            \toprule
             Train DB & \multicolumn{2}{c}{CLIVE} & \multicolumn{2}{c}{KonIQ} & \multicolumn{2}{c}{SPAQ}\\
            \midrule
             Test DB & KonIQ & SPAQ & CLIVE & SPAQ & CLIVE & KonIQ \\
            \midrule
            HyperIQA & 0.772 & 0.854 & 0.785 & 0.824 & 0.737 & 0.732\\
            CONTRIQUE & 0.676 & 0.842 & 0.731 & 0.789 & 0.549 & 0.646 \\
            Re-IQA & 0.769 & 0.852 & 0.791 & 0.862 & 0.732 & 0.707\\
            CLIP & 0.725 & 0.850 & 0.799 & 0.837 & 0.773 & \underline{0.753} \\
            CLIP-IQA+ & 0.697 & 0.836 & 0.803 & 0.832 & \underline{0.784} & 0.722 \\
            LIQE & \underline{0.819} & \underline{0.877} & \underline{0.824} & \underline{0.868} & - & - \\
            \midrule
            ATTIQA & \textbf{0.829} & \textbf{0.887} & \textbf{0.856} & \textbf{0.879} & \textbf{0.824} & \textbf{0.819} \\
            \bottomrule
            \end{tabular}
        }
        \label{table:cv}
        \end{minipage}
\end{table}


==> Main/partials/table_lp.tex <==
\begin{table}[t]
\label{t3}
\begin{center}
\resizebox{\columnwidth}{!}
{
    \begin{tabular}{c||cc|cc|cc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c}{CLIVE} & \multicolumn{2}{c}{KonIQ} & \multicolumn{2}{c}{SPAQ}\\
    & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
    \midrule
    CONTRIQUE & \underline{0.845} & \underline{0.857} & 0.894 & 0.906 & \underline{0.916} & 0.919 \\
    QPT & 0.761 & 0.794 & - & - & - & -\\
    Re-IQA (quality) & 0.806 & 0.824 & 0.861 & 0.885 & 0.900 & 0.910 \\
    Re-IQA (content) & 0.808 & 0.844 & 0.896 & 0.912 & 0.902 & 0.908 \\
    Re-IQA (both) & 0.840 & 0.854 & \textbf{0.914} & \textbf{0.923} & \textbf{0.918} & \textbf{0.925} \\
    CLIP & 0.803 & 0.829 & 0.883 & 0.895 & 0.895 & 0.896 \\
    \midrule
    ATTIQA & \textbf{0.870} & \textbf{0.891} & \underline{0.903} & \underline{0.918}  & \textbf{0.918} & \underline{0.922} \\
    \bottomrule
    \end{tabular}
}
\end{center}
\caption{Linear probing performance comparison of ATTIQA and NR-IQA methods which focuses on representation learning.}
\label{table:lp}
\end{table}

==> Main/partials/table_lp_ablation.tex <==
\begin{table}[htb]
\centering
\caption{(a) Personal IQA performance comparison of ATTIQA and existing NR-IQA methods. (b) Ablation study results.}
\subfloat[Personal IQA Adaptation]{%
\resizebox{0.49\columnwidth}{!}{
      \begin{tabular}{c||cc|cc|cc}
        \toprule
        \multirow{2}{*}{Prompt type}& \multicolumn{2}{c}{GIQA} & \multicolumn{2}{c}{zero-shot PIQA} & \multicolumn{2}{c}{fine-tuned PIQA}\\
        & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
        \midrule
        HyperIQA & 0.867 & 0.919 & 0.622 & \underline{0.703} & 0.629 & 0.726 \\
        CONTRIQUE & 0.849 & 0.897 & \underline{0.625} & 0.679 & 0.647 & 0.693  \\
        Re-IQA & 0.885 & 0.931 & 0.619 & 0.688 & \underline{0.657} & \underline{0.741} \\
        CLIP & \underline{0.892} & \underline{0.934} & - & - & - & - \\
        CLIP-IQA+ & 0.860 & 0.904 & - & - & - & - \\
        \midrule
        ATTIQA & \textbf{0.906} & \textbf{0.941} & \textbf{0.653} & \textbf{0.726} & \textbf{0.689} & \textbf{0.767}  \\
        \bottomrule
        \end{tabular}
    }
}
\subfloat[Ablation Studies]{%
    \resizebox{0.48\columnwidth}{!}{
        \begin{tabular}{c||cc|cc|cc}
    \toprule
    \multirow{2}{*}{Prompt type}& \multicolumn{2}{c}{CLIVE} & \multicolumn{2}{c}{KonIQ} & \multicolumn{2}{c}{SPAQ}\\
    & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
    \midrule
    ATTIQA & \textbf{0.898} & \textbf{0.916} & \textbf{0.942} & \textbf{0.952} & \textbf{0.926} & \textbf{0.930} \\
    \midrule
    single-prompt & 0.880 & 0.909 & 0.928 & 0.939 & 0.916 & 0.920 \\
    \midrule
    Worst prompt & 0.869 & 0.889 & 0.930 & 0.943 & 0.920 & 0.925 \\
    Median prompt & 0.872 & 0.893 & 0.931 & 0.944 & 0.921 & 0.925 \\
    % Hand-crafted & 0.896 & 0.914 & 0.940 & 0.950 & 0.925 & 0.929 \\
    \midrule
    with $L_2$ &  0.875 & 0.904 & 0.933 & 0.945 & 0.923 & 0.928 \\  
    \bottomrule
    \end{tabular}
    }
}
\label{table:piqa_ablation}
\end{table}

==> Main/partials/table_piqa.tex <==
\begin{table}[t]

\label{t3}
\begin{center}
\resizebox{\columnwidth}{!}
{
        \begin{tabular}{c||cc|cc|cc}
    \toprule
    \multirow{2}{*}{Prompt type}& \multicolumn{2}{c}{GIQA} & \multicolumn{2}{c}{zero-shot PIQA} & \multicolumn{2}{c}{fine-tuned PIQA}\\
    & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
    \midrule
    HyperIQA & 0.867 & 0.919 & 0.622 & \underline{0.703} & 0.629 & 0.726 \\
    CONTRIQUE & 0.849 & 0.897 & \underline{0.625} & 0.679 & 0.647 & 0.693  \\
    Re-IQA & \underline{0.885} & \underline{0.931} & 0.619 & 0.688 & \underline{0.657} & \underline{0.741} \\
    \midrule
    ATTIQA & \textbf{0.906} & \textbf{0.941} & \textbf{0.653} & \textbf{0.726} & \textbf{0.689} & \textbf{0.767}  \\
    \bottomrule
    \end{tabular}
}
\end{center}
\caption{Personal IQA performance comparison of ATTIQA and existing NR-IQA methods.}
\label{table:piqa}
\end{table}

==> Main/partials/table_prompt.tex <==
\begin{table}[t]

\label{t3}
\begin{center}
\resizebox{\columnwidth}{!}
{


    \begin{tabular}{c||cc|cc|cc}
    \toprule
    \multirow{2}{*}{Prompt Criterion}& \multicolumn{2}{c}{CLIVE} & \multicolumn{2}{c}{KonIQ} & \multicolumn{2}{c}{SPAQ}\\
    & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
    \midrule
    Single prompt & 0.880 & 0.909 & 0.928 & 0.939 & 0.916 & 0.920 \\
    \midrule
    Randomly selected & 0.898 & 0.914 & 0.940 & 0.951 & 0.925 & 0.929 \\
    Distortion Intensity & 0.891 & 0.910 & 0.929 & 0.943 & 0.922 & 0.926 \\
    Human Interpretation & 0.890 & 0.915 & \textbf{0.942} & \textbf{0.952} & 0.925 & \textbf{0.930} \\
    \midrule
    Mixed & \textbf{0.898} & \textbf{0.916} & \textbf{0.942} & \textbf{0.952} & \textbf{0.926} & \textbf{0.930} \\
    \bottomrule
    \end{tabular}


}
\end{center}
\caption{Accuracy between human preference and IQA model for images generated from generative models.}
\label{table:ablation_prompt}
\end{table}


    % \begin{tabular}{c||cc|cc|cc}
    % \toprule
    % \multirow{2}{*}{Prompt Criterion}& \multicolumn{2}{c}{CLIVE} & \multicolumn{2}{c}{KonIQ} & \multicolumn{2}{c}{SPAQ}\\
    % & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC \\
    % \midrule
    % Base Prompt & 0.880 & 0.905 & 0.932 & \underline{0.947} & \underline{0.922} & 0.927 \\
    % KADID-10k & 0.863 & 0.893 & 0.926 & 0.942 & 0.921 & 0.925 \\
    % SPAQ & \underline{0.885} & \underline{0.908} & \textbf{0.934} & \textbf{0.947} & \underline{0.922} & \underline{0.927} \\
    % \bottomrule
    % ATTIQA & \textbf{0.887} & \textbf{0.912} & \textbf{0.934} & 0.946 & \textbf{0.923} & \textbf{0.927} \\
    % \bottomrule
    % \end{tabular}

==> Rebuttal/partials/attribute_analysis.tex <==
\begin{figure}[t]
\centering
\includegraphics[clip, trim={
70pt 3pt 0 0}, width=1\columnwidth]{Rebuttal/partials/attribute_analysis.pdf}
\vspace{-18pt}
\caption{Correlation graph illustrating the relationship between MOS and Grad-CAM across varying intensity of image attributes.}
\label{fig:attribute_analysis}
\vspace{-18pt}
\end{figure}

==> Rebuttal/partials/table_another.tex <==
\begin{table}[!t]
\centering
\vspace{-15pt}
\begin{minipage}{0.53\linewidth}
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{c||cc|cc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c}{FLIVE} & \multicolumn{2}{c}{AVA} \\
    & SROCC & PLCC& SROCC & PLCC\\
    \midrule
    DBCNN & 0.542 & 0.626 & 0.554 & 0.583 \\
    CLIP-IQA+ & 0.575 & 0.593 & 0.692 & 0.732 \\
    \midrule
    ATTIQA & \textbf{0.632} & \textbf{0.732} & \textbf{0.761} & \textbf{0.761} \\
    \bottomrule
    \end{tabular}
}
\vspace{-9pt}
\caption{Table 2 Supplement}
\label{table:another_1}
\end{minipage}%
\hfill
\begin{minipage}{0.45\linewidth}
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{c||ccc}
    \toprule
    Train DB & \multicolumn{3}{c}{FLIVE}\\
    \midrule
    Test DB & CLIVE & KonIQ & SPAQ\\
    \midrule
    CLIP-IQA+ & 0.620 & 0.631 & 0.661 \\
    \midrule
    ATTIQA & \textbf{0.756} & \textbf{0.762} & \textbf{0.867}  \\
    \bottomrule
    \end{tabular}
}
\vspace{-9pt}
\caption{Table 3 Supplement}
\label{table:another_2}
\end{minipage}
\vspace{-18pt}
\end{table}



% \begin{table}[!htb]
% \label{t3}
% \begin{center}
% \resizebox{\columnwidth}{!}
% {
%     \begin{tabular}{c||cc|cc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multicolumn{2}{c}{FLIVE} & \multicolumn{2}{c}{AVA} \\
%     & SROCC & PLCC& SROCC & PLCC\\
%     \midrule
%     DBCNN & 0.962 & 0.966 & 0.923 & 0.942 \\
%     CLIP-IQA+ & 0.896 & 0.914 & 0.940 & 0.950 \\
%     \midrule
%     ATTIQA & \textbf{0.898} & \textbf{0.916} & \textbf{0.942} & \textbf{0.952} \\
%     \bottomrule
%     \end{tabular}
% }
% \end{center}
% \vspace{-8pt}
% \caption{Performance comparison fon IQA Dataset with Synthetic Distortions.}
% \label{table:synthetic}
% \vspace{-12pt}
% \end{table}

% \begin{table}[!tb]

% \centering
% \vspace{-12pt}
% \subfloat[Supplementary of Table 2]{%
% \resizebox{0.52\columnwidth}{!}{
%     \begin{tabular}{c||cc|cc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multicolumn{2}{c}{FLIVE} & \multicolumn{2}{c}{AVA} \\
%     & SROCC & PLCC& SROCC & PLCC\\
%     \midrule
%     DBCNN & 0.542 & 0.626 & 0.554 & 0.583 \\
%     CLIP-IQA+ & 0.575 & 0.593 & 0.692 & 0.732 \\
%     \midrule
%     ATTIQA & \textbf{0.632} & \textbf{0.732} & \textbf{0.761} & \textbf{0.761} \\
%     \bottomrule
%     \end{tabular}
% }
% }
% \subfloat[Supplementary of Table 3]{%
%     \resizebox{0.45\columnwidth}{!}{
%     \begin{tabular}{c||ccc}
%     \toprule
%     Train DB & \multicolumn{3}{c}{FLIVE}\\
%     \midrule
%     Test DB & CLIVE & KonIQ & SPAQ\\
%     \midrule
%     CLIP-IQA+ & 0.620 & 0.631 & 0.661 \\
%     \midrule
%     ATTIQA & \textbf{0.756} & \textbf{0.762} & \textbf{0.867}  \\
%     \bottomrule
%     \end{tabular}
% }
% }
% \label{table:another}
% \vspace{-20pt}
% \end{table}


% {
%     \begin{tabular}{c||cc|cc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multicolumn{2}{c}{FLIVE} & \multicolumn{2}{c}{AVA} \\
%     & SROCC & PLCC& SROCC & PLCC\\
%     \midrule
%     DBCNN & 0.542 & 0.626 & 0.554 & 0.583 \\
%     CLIP-IQA+ & 0.575 & 0.593 & 0.692 & 0.732 \\
%     \midrule
%     ATTIQA & \textbf{0.632} & \textbf{0.732} & \textbf{0.761} & \textbf{0.761} \\
%     \bottomrule
%     \end{tabular}
% }

==> Rebuttal/partials/table_attribute.tex <==
\begin{table}[t]
\label{t3}
\begin{center}
\resizebox{0.95\columnwidth}{!}
{
    \begin{tabular}{c||cc|cc|cc|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{Sharpness} & \multicolumn{2}{c}{Contrast} & \multicolumn{2}{c}{Brightness} & \multicolumn{2}{c}{Colorfulness} & \multicolumn{2}{c}{Noisiness} & \multicolumn{2}{c}{ATTIQA}\\
    & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC  \\
    \midrule
    CLIVE & 0.890 & 0.910 & 0.870 & 0.905 & 0.880 & 0.905 & 0.881 & 0.906 & 0.878 & 0.901 & \textbf{0.898} & \textbf{0.916} \\
    KonIQ & 0.939 & 0.950 & 0.937 & 0.947 & 0.936 & 0.948 & 0.934 & 0.945 & 0.939 & 0.950 & \textbf{0.942} & \textbf{0.951} \\
    SPAQ & 0.925 & 0.929 & 0.923 & 0.928 & 0.923 & 0.926 & 0.924 & 0.927 & 0.924 & 0.928 & \textbf{0.926} & \textbf{0.930} \\
    \bottomrule
    \end{tabular}
}
\vspace{-9pt}
\caption{performance comparison of fine-tuning which only utilizes ATTIQA's each attribute head.}
\label{table:attribute}
\end{center}
\vspace{-25pt}

\end{table}




==> Rebuttal/partials/table_feature.tex <==


\begin{table}[t]
\vspace{-12pt}
\label{t3} % here
\centering
\resizebox{0.9\columnwidth}{!}
{
    \centering
    \begin{tabular}{c||c|c|c}
    \toprule
     Fine-tune DB & CLIVE & KonIQ & SPAQ\\
    % \midrule
    %  Test DB & CLIVE & KonIQ & SPAQ & CLIVE & KonIQ & SPAQ & CLIVE & KonIQ & SPAQ \\
    \midrule
    \makecell{CLIP \\ (cosine similarity btw original $\leftrightarrow$ finetuned CLIP)} & 0.195 & 0.203  & 0.309\\
    \midrule
    \makecell{ATTIQA \\ (cosine similarity btw pretrained $\leftrightarrow$ finetuned ATTIQA)} & 0.890 & 0.811 & 0.945\\
    \bottomrule
    \end{tabular}  
}
\vspace{-8pt}
\caption{
% Cosine similarity between features from pretrained and fine-tuned encoder.
A good generalization ability (\ie high cosine similarity) for IQA is obtained through our pretraining.}
\vspace{-3mm}
\label{table:feature} % here
\end{table}

% {
%     \centering
%     \begin{tabular}{c||ccc|ccc|ccc}
%     \toprule
%      Fine-tune DB & \multicolumn{3}{c}{CLIVE} & \multicolumn{3}{c}{KonIQ} & \multicolumn{3}{c}{SPAQ}\\
%     % \midrule
%     %  Test DB & CLIVE & KonIQ & SPAQ & CLIVE & KonIQ & SPAQ & CLIVE & KonIQ & SPAQ \\
%     \midrule
%     CLIP & 0.195 & 0.203 & 0.309 & 0.225 & 0.209 & 0.307 & 0.242 & 0.277 & 0.341\\
%     \midrule
%     ATTIQA & 0.011 & 0.012 & 0.012 & 0.011 & 0.009 & 0.010 & -0.025 & -0.021 & -0.026\\
%     \bottomrule
%     \end{tabular}  
% }


==> Rebuttal/partials/table_liqe.tex <==
\begin{table}[t]
\label{t3}
\begin{center}
\resizebox{0.95\columnwidth}{!}
{
    \begin{tabular}{c|c||c|c|c|c|c|c||c|c|c}
    \toprule
    &\multirow{2}{*}{Methods} & \multicolumn{6}{c}{Seen Dataset} & \multicolumn{3}{c}{Unseen Dataset} \\
    &&LIVE & CSIQ & KADID & BID & LIVEC & KonIQ & TID & SPAQ & PIPAL\\
    \midrule
    SR& LIQE & 0.970 & \textbf{0.936} & \textbf{0.930} & 0.875 & \textbf{0.904} & 0.919 & \textbf{0.811} & 0.881 & 0.478 \\
    CC&ATTIQA & \textbf{0.974} & \textbf{0.936} & 0.923 & \textbf{0.891} & 0.901 & \textbf{0.920} & 0.796 & \textbf{0.891} & \textbf{0.521}\\
    \midrule
    PL&LIQE & 0.951 & 0.939 & \textbf{0.931} & 0.900 & 0.910 & 0.908 & - & - & - \\
    CC&ATTIQA & \textbf{0.977} & \textbf{0.950} & 0.927 & \textbf{0.918} & \textbf{0.917} & \textbf{0.932} & - & - & -\\
    \bottomrule
    \end{tabular}
}
\vspace{-9pt}
\caption{Performance comparison with LIQE.}
\label{table:liqe}
\end{center}
\vspace{-21pt}
\end{table}


==> Rebuttal/partials/table_method.tex <==

\begin{table}[!htb]
\vspace{-12pt}
\label{t3}
\begin{center}
\resizebox{\columnwidth}{!}
{
    \begin{tabular}{c||c|c|c|c}
    \toprule
    Methods & QPT & LIQE & CLIP-IQA+ & \textbf{ATTIQA} \\
    \midrule
    \makecell{Quality-Aware \\  Pretraining} & \faCircleThin & \ding{53} & \ding{53} & \faCircleThin\\
    \midrule
    \makecell{VLM Strategy \\  (used stage)} & \ding{53} & \makecell{Optimize whole CLIP \\ (fine-tune stage)} & \makecell{Optimize CLIP prompt \\ (fine-tune stage)} & \makecell{\textbf{Generate pseudo-label} \\ \textbf{(pretrain stage)}}\\
    \midrule
    % VLM Knowledge & \ding{53}& \bigcirc & \bigcirc & \faCircleThin \\
    Backbone & ResNet-50 & CLIP & CLIP & \textbf{ResNet-50} \\
    \bottomrule
    \end{tabular}
}
\end{center}
\vspace{-18pt}
\caption{Differences among ATTIQA and existing works.}
\vspace{-15pt}
\label{table:method}
\end{table}


% {
%     \begin{tabular}{c||c|c|c}
%     \toprule
%     Methods & \makecell{Quality-Aware \\  Pretraining} & \makecell{VLM \\ Knowledge} & VLM Usage \\
%     \midrule
%     QPT & \faCircleThin & \ding{53} & - \\
%     \midrule
%     LIQE & \ding{53}& \faCircleThin & \makecell{Optimize CLIP itself \\ (fine-tune stage)} \\
%     \midrule
%     CLIP-IQA & \ding{53} & \faCircleThin & \makecell{Optimize prompt \\ (fine-tune stage)} \\
%     \midrule
%     ATTIQA & \faCircleThin & \faCircleThin & \makecell{Generate pseudo-label \\ (pretrain stage)} \\
%     \bottomrule
%     \end{tabular}
% }

==> Rebuttal/partials/table_synthetic.tex <==
\begin{table}[!tb]
\label{t3}
\begin{center}
\resizebox{0.95\columnwidth}{!}
{
    \begin{tabular}{c||cc|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c}{LIVE} & \multicolumn{2}{c}{CSIQ} & \multicolumn{2}{c}{TID2013} & \multicolumn{2}{c}{KADID-10k}\\\
    & SROCC & PLCC& SROCC & PLCC& SROCC & PLCC & SROCC & PLCC\\
    \midrule
    CONTRIQUE & 0.962 & 0.964 & 0.945 & \textbf{0.955} & \underline{0.885} & \underline{0.883} & \textbf{0.919} & \textbf{0.919} \\
    Re-IQA & 0.966 & 0.968 & \underline{0.946} & \textbf{0.955} & 0.877 & \underline{0.883} & 0.912 & 0.910 \\
    CLIP & \underline{0.968} & \underline{0.970} & 0.944 & 0.934 & 0.858 & 0.858 & 0.898 & 0.897 \\
    CLIP-IQA+ & 0.919 & 0.922 & 0.886 & 0.899 & 0.856 & 0.862 & 0.792 & 0.790 \\
    \midrule
    ATTIQA & \textbf{0.970} & \textbf{0.972} & \textbf{0.948} & \underline{0.953} & \textbf{0.898} & \textbf{0.903} & \underline{0.917} & \underline{0.917} \\
    \bottomrule
    \end{tabular}
}
\end{center}
\vspace{-18.5pt}
\caption{Performances on Synthetic Distortion IQA Dataset}
\label{table:synthetic}
\vspace{-10pt}
\end{table}
